Associators from an operadic point of view

This is a survey on Drinfeld associators and their generalizations, where we focus on operadic aspects.

==> hello.tex <==
%Comments by me

\newcommand{\Victor}[1]{\textcolor{blue}{#1}}


\newcommand{\colim}[1]{\underset{#1}{\mathrm{colim}}~}

% Symbols

\newcommand{\kk}{\Bbbk}
\newcommand{\ac}{\scriptstyle \textrm{!`}}
\newcommand{\iso}{\ \raisebox{0.5ex}{\ensuremath{\stackrel{\sim}{\rule{16pt}{0.7pt}}}\ \,}}
\newcommand{\qi}{\xrightarrow{
   \,\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\,}}
  
%Yoneda Embedding

\newcommand{\yo}{\begin{CJK}{UTF8}{ipmxa}\textbf{よ}\end{CJK}}

%Categories

\newcommand{\smod}{\mathbb{S}\text{-}\mathsf{mod}}

%Operads

\newcommand{\cob}{\mathcal{C}o\mathcal{B}}
\newcommand{\pab}{\mathcal{P}a\mathcal{B}}
\newcommand{\pacd}{\mathcal{P}a\mathcal{CD}}
